Deeper Insights into Weight Sharing in Neural Architecture Search

With the success of deep neural networks, Neural Architecture Search (NAS) as a way of automatic model design has attracted wide attention. As training every child model from scratch is very time-consuming, recent works leverage weight-sharing to speed up the model evaluation procedure. These approaches greatly reduce computation by maintaining a single copy of weights on the super-net and share the weights among every child model. However, weight-sharing has no theoretical guarantee and its impact has not been well studied before. In this paper, we conduct comprehensive experiments to reveal the impact of weight-sharing: (1) The best-performing models from different runs or even from consecutive epochs within the same run have significant variance; (2) Even with high variance, we can extract valuable information from training the super-net with shared weights; (3) The interference between child models is a main factor that induces high variance; (4) Properly reducing the degree of weight sharing could effectively reduce variance and improve performance.

==> discussion.tex <==
\section{Discussion}

Though the insights are from a down-scaled search space, we believe most of them still hold in large search spaces. These insights, to some extent, echo some previous research works on weight-sharing-based NAS, \eg ENAS and DARTS, which use RL controller and differentiable architecture weights respectively, to alleviate the interference among child models. According to our experiments, they could find a child model with acceptable, but still show high instability. To further improve NAS, we believe the key is to figure out how to smartly leverage shared weights. This paper suggests controlling the degree of weight-sharing, either model-based and rule-based, evaluating them on the small search space and providing deeper insights. We hope to inspire the community to find more stable yet efficient approaches.


==> prefix_sharing.tex <==
\subsection{Prefix Sharing}

Inspired by the great success of transfer learning~\cite{caruana1995learning,mesnil2011unsupervised,kornblith2019better}, we try to do a similar thing by sharing one copy of ``backbone'' network while keeping a separated copy of ``head'' for each child model. We adopt a similar strategy as weight sharing to train child models in a supernet in turn, but keep an independent copy of unshared parameters for each child model, so that updating one child model won't affect others for these parameters.

We only share parameters in some cells at the bottom of the network. In particular, we use $k$ to denote the number of cells shared. When $k=0$, only the first two conv layers are shared. When $k=4$, all the layers except the final fully-connected layers are shared. Since sharing part of weights will serialize the training (as opposed to parallelizing the groups in \S\ref{sec:group-sharing}), we increase the total epochs from $200$ to $2000$. Results are shown in \autoref{tab:prefix-sharing-gt-tau}.

\begin{table}[htbp]
    \centering
    \caption{GT-Tau (mean, std) and accuracy (mean, std) evaluated for the last $64$ mini-batches. Accuracy of each child model in each instance is first averaged over $64$ mini-batches, then mean and std for these $64$ values in an instance are calculated. Then we average this over $10$ instances. The subscript is the standard variance of the corresponding average.}
    \label{tab:prefix-sharing-gt-tau}
    \small
    \begin{tabular}{ccccc}
    \toprule
    $k$ & GT-Tau-Mean-64 & GT-Tau-Std-64 & Accuracy Mean & Accuracy Std \\
    \midrule
    $0$ & $0.7250 _{\pm 0.0366}$ & $0.0122 _{\pm 0.0026}$ & $0.7790 _{\pm 0.0025}$ & $0.0247 _{\pm 0.0004}$ \\
    $1$ & $0.5250 _{\pm 0.0155}$ & $0.0649 _{\pm 0.0131}$ & $0.7705 _{\pm 0.0064}$ & $0.0378 _{\pm 0.0017}$ \\
    $2$ & $0.4154 _{\pm 0.0447}$ & $0.1546 _{\pm 0.0227}$ & $0.6879 _{\pm 0.0369}$ & $0.0793 _{\pm 0.0280}$ \\
    $3$ & $0.4137 _{\pm 0.0219}$ & $0.1628 _{\pm 0.0258}$ & $0.6513 _{\pm 0.0159}$ & $0.0753 _{\pm 0.0070}$ \\
    $4$ & $0.4891 _{\pm 0.0219}$ & $0.1705 _{\pm 0.0124}$ & $0.6542 _{\pm 0.0077}$ & $0.1035 _{\pm 0.0143}$ \\
    \bottomrule
    \end{tabular}
\end{table}

Obviously, sharing fewer layers improves the GT-Tau and accuracy (from $0.65$ on average in $k=4$ to $0.78$ in $k=0$), at the cost of consuming more computation power of course. Although the high and stable GT-Tau obtained when $k=0$, it takes over 1000 epochs for it to climb up to above $0.6$. However, this cost is still way much lower than ground truth, which takes $64 \times 200 = 12800$ epochs in total, despite the great acceleration brought by parallelizing these $64$ runs.

